Extremal Property of the Square Lattice

Motivated by a 2019 result of Faulhuber-Steinerberger, we demonstrate that the real square lattice $\mathbb{Z}^2$ exhibits the same local, extremal property as the hexagonal lattice $\Lambda$, where distances of lattice points from the `deep holes' of natural fundamental domains increase under perturbation. If $\Delta$ is a small perturbation of $\mathbb{Z}^2$ in the space of unimodular lattices, consider $C_r$, the set of points in $A_r$ shifted to $\Delta$. If $\Delta$ is a perturbation of the lattice $\mathbb{Z}^2$ with respect to the Euclidean metric, then for a fixed deep hole $p$, the summed total distance of lattice points to $p$ strictly increases, and is bounded below by a function of the distance between the lattice and its perturbation. Additionally, we show this growth is approximately preserved by convex functions.

==> bib.bib.tex <==


 @article{extremal,
 author={Steinerberger, Stefan and Faulhuber, Markus},
   title={An Extremal Property of the Hexagonal Lattice},
   volume={177},
   ISSN={1572-9613},
   url={http://dx.doi.org/10.1007/s10955-019-02368-3},
   DOI={10.1007/s10955-019-02368-3},
   number={2},
   journal={Journal of Statistical Physics},
   publisher={Springer Science and Business Media LLC},
   year={2019},
   month={Aug},
   pages={285–298}
}

@book{spheres, 
    title={Sphere Packings, Lattices and Groups}, 
  %  %volume={}, 
    ISBN={978-0-387-98585-5},
    %DIO={10.1007/978-1-4757-2016-7},
    %number={}
    journal={Grundlehren der Mathematischen Wissenschaften}, 
    publisher={Springer-Verlag},
    author={Conway, John and Sloane, Neil },
    year={1999}, 
    %month={}, 
    pages={290 (3rd ed.)}
}


@article{unimodular,
   title={Unimodular Lattices, Together With A Table of the Best Such Lattices},
   volume={177},
   %ISSN={1572-9613},
   %url={http://dx.doi.org/10.1007/s10955-019-02368-3},
  % DOI={10.1007/s10955-019-02368-3},
   number={2},
   journal={Catalog of Lattices},
   publisher={Online},
   author={Nebe, Gabriele and Sloane, Neil },
   year={2015},
   month={May},
   pages={285–298}
}



%[K] Shmuel Kantorovitz, Introduction to Modern Analysis. Oxford Graduate Texts in Mathematics, 8. Oxford
%University Press, Oxford, 2003.   
% @book{SK,
%   title={Introduction to Modern Analysis},
   %volume={},
%   ISBN={9780199203154},
   %journal={},
%   publisher={Oxford Graduate Texts in Mathematics},
 %  author={Kantorovitz, Shmuel},
 %  year={2003}
%}
   
%[MZ] D. Montgomery and L. Zippin, Topological Transformation Groups. Interscience Publishers, New York-London, 1955.   


@article{M.Z.,
   title={Topological Transformation Groups},
   volume={41},
   DOI={10.2307/1968858},
   number={4},
   journal={Annals of Mathematics},
   author={ Montgomery, Denae and Zippin, Leo},
   year={1940}
 }  

  

 @book{RV,
   title={Fourier Analysis on Number Fields},
   ISBN={978-1-4757-3085-2},
   journal={Graduate Texts in Mathematics},
   publisher={Springer-Verlag},
   author={Ramakrishnan,   Dinakar and Valenza, Robert J. },
   year={1999}
}
   
%[M] J.R. Munkres, Topology: a first course. Prentice-Hall, Inc., Englewood Cli↵s, N.J., 1975.   
 %@book{Munkres,
  % title={Topology: a first course},
   %ISSN={0139254951 9780139254956},
   %publisher={Prentice-Hall, Inc.},
   %author={Munkres, J. R. },
   %year={1975}
 %}
 



@article{LatBase,
    author = {Micciancio, Daniele  and Regev, Oded },
    title = {Lattice-based cryptography},
    year = {2008}
}


%@article{Notes1, 
 %   author = {Remi Boutonnet},
  %  title = {Lattices in semi-simple Lie groups},
   % publisher = {CIRM},
    %year = {2020}
%}

%@article{bary,
 %   author = {Jean Meeus}, 
  %  date = {1997}, 
   % publisher = {Mathematical Astronomy Morsels, Willmann-Bell},
    %pages ={165–168}, 
    %ISBN =  {0-943396-51-4}
%}

@article{LatLie,
  title={Five Lectures on Lattices in Semisimple Lie Groups},
  author={Yves Benoist et. all},
  journal={fill in},
  year={2006}
}


@book{Rudin, 
    title={Real and Complex Analysis}, 
    author={ Rudin, Walter},
    number={Third edition},
    publisher={McGraw-Hill Book Co.},
    date={1987}
}

@article{haar,
title = {An example of arithmetic groups}, 
author = {Michler, Sebastian },
publisher = {online}, 
date = {2016}

}

@article{quasi, 
author= {Lagarias, J. C.},
title= {Meyer's concept of quasicrystal and quasiregular sets}, 
journal = {Comm. Math. Phys.}, 
number = {179},
date = {1996},
pages = {365–376}
}

@article{holonomy,
author = {Hubert, Pascal and Schmidt, Thomas},
year = {2006},
month = {01},
title = {An Introduction to Veech Surfaces},
journal = {Handbook of Dynamical Systems, vol. 1B}
}

@article{penrose,
author = { Mackay, Alan L.},
title = {Crystallography and the Penrose pattern},
journal = {Physica A: Statistical Mechanics and its Applications},
volume ={114}, 
date = {1982},
pages ={609-613},
ISSN ={0378-4371}
}

@article{tilings,
author = {Branko and Grunbaum and Shephard},
title={Tilings by Regular Polygons},
journal={Mathematics Magazine}, 
volume={ 50}, 
publisher={Mathematical Association of America},
date={1977},
pages={227–247}, 
doi={10.2307/2689529}
}


%@article{hales_adams_bauer_dang_harrison_hoang_kaliszyk_magron_mclaughlin_nguyen_et al._2017, 
%title={A FORMAL PROOF OF THE KEPLER CONJECTURE}, 
%volume={5}, 
%DOI={10.1017/fmp.2017.1}, 
%journal={Forum of Mathematics, Pi}, 
%publisher={Cambridge University Press}, 
%author={HALES, THOMAS and ADAMS, MARK and BAUER, GERTRUD and DANG, TAT DAT and HARRISON, JOHN and HOANG, LE TRUONG and KALISZYK, CEZARY and MAGRON, VICTOR and MCLAUGHLIN, SEAN and NGUYEN, TAT THANG and et al.}, 
%year={2017}, 
%pages={e2}}

@book{crypto,
author = {Hoffstein and Pipher and Silverman},
title={An Introduction to Mathematical Cryptography},
number={First edition},
publisher={Springer New York, NY},
date={2008} ,
ISBN={978-1-4419-2674-6},
DOI={https://doi.org/10.1007/978-0-387-77993-5}
}

@article{groupslattices,
author={R. Schmidt},
title={Subgroup Lattices of Groups},
edition={14},
journal={de Gruyter Expositions in Mathematics},
publisher={Walter de Gruyter and Co., Berlin},
date={1994}
}

@article{reptheorylat,
author={A. Lucchini}, 
title={Representation of certain lattices as intervals in subgroup lattices},
publisher = {J. Algebra},
number={164}, 
date={1994}, 
pages={85–90}
}
